Teleoperator Imitation with Continuous-time Safety

Learning to effectively imitate human teleoperators, with generalization to unseen and dynamic environments, is a promising path to greater autonomy enabling robots to steadily acquire complex skills from supervision. We propose a new motion learning technique rooted in contraction theory and sum-of-squares programming for estimating a control law in the form of a polynomial vector field from a given set of demonstrations. Notably, this vector field is provably optimal for the problem of minimizing imitation loss while providing continuous-time guarantees on the induced imitation behavior. Our method generalizes to new initial and goal poses of the robot and can adapt in real-time to dynamic obstacles during execution, with convergence to teleoperator behavior within a well-defined safety tube. We present an application of our framework for pick-and-place tasks in the presence of moving obstacles on a 7-DOF KUKA IIWA arm. The method compares favorably to other learning-from-demonstration approaches on benchmark handwriting imitation tasks.

==> comparison_table.tex <==
%{\bf Angle}
%
\scriptsize
%\begin{figure*}
%\centering
%\begin{minipage}[t]{0.45\linewidth}\centering
%\begin{table*}[ht]
%\scriptsize
\begin{tabular}{|c|c|c|c H H}       
\hline
Metric & DMP & SEDS & CLFDM & CVF-CF & CVF-GS \\                  
\hline                                                                
TrainingTrajectoryError & 4.10 & 7.18 & 4.93 & 6.70 & 5.84 \\         
\hline                                                                
TrainingVelocityError & 7.40 & 14.62 & 10.99 & 17.70 & 15.25 \\       
\hline                                                                
TestTrajectoryError & 5.53 & 4.58 & 12.24 & 6.09 & 4.16 \\            
\hline                                                                
TestVelocityError & 8.74 & 11.43 & 15.50 & 15.50 & 13.01 \\           
%\hline                                                                
%TrainingDTWD & 2197.60 & 3929.72 & 2406.22 & 2474.13 & 1982.40 \\     
%\hline                                                                
%TestDTWD & 2350.49 & 2837.70 & 6883.36 & 3332.69 & 2551.86 \\         
%\hline                                                                
\hline                                                                
DistanceToGoal & 3.59 & 3.25 & 6.70 & 6.65 & 3.99 \\                  
\hline                                                                
DurationToGoal & - & 3.89 & 4.34 & 4.76 & 3.50 \\                     
\hline                                                                
NumberReachedGoal & 0.00 & 7.00 & 7.00 & 7.00 & 7.00 \\               
\hline                                                                
%TrainingDTWD@30T & 47277.90 & 3719.13 & 2185.27 & 1606.84 & 1404.78 \\
%\hline                                                                
%TestDTWD@30T & 54955.18 & 2883.74 & 4082.38 & 2370.18 & 2092.40 \\    
%\hline                                                                
GridDuration & 5.91 & 3.72 & 9.73 & 3.40 & 2.41 \\                    
\hline                                                                
GridFractionReachedGoal & 0.06 & 1.00 & 1.00 & 1.00 & 1.00 \\         
\hline                                                                
GridDistanceToGoal & 3.33 & 1.00 & 1.00 & 1.00 & 1.00 \\              
\hline               
GridDTWD & 24493.27 & 13865.75 & 14503.13 & 11311.29 & 8865.90 \\     
\hline  
TrainingTime & 0.05 & 2.10 & 2.82 & 7.58 & 3.29 \\ 
\hline
IntegrationSpeed & 0.21 & 0.06 & 0.15 & 0.15 & 0.04 \\ 
\hline
\end{tabular}% 
\begin{tabular}{H H}
     \hline
     CVF-CF & CVF-GS \\
     \hline
     5.44 & 5.21 \\
     \hline
     11.92 & 10.45 \\
     \hline
     4.17 & 3.19 \\
     \hline
     11.27 & 9.05 \\
     \hline
     3.69 & 2.04 \\
     \hline
     3.29 & 3.01 \\
     \hline
     7.00 & 7.00 \\
     \hline
     1.73 & 2.30 \\
     \hline
     1.00 & 1.00 \\
     \hline
     1.00 & 1.00 \\
     \hline
     12837.89 & 9451.88 \\
     \hline
     23.64 & 23.90 \\
     \hline
     0.04 & 0.04 \\
     \hline
     \end{tabular}%
\Anglestats
%\end{minipage}%
%\begin{minipage}[t]{0.5\linewidth}
%\hspace{0.8cm}
%\begin{figure}
 %   \centering
 %   \vspace{-0.5cm}\includegraphics[height=5cm]{img/grid-dtwd.png}
%    \caption{Caption}
%    \label{fig:my_label}
%\end{figure}
%  $$\scriptsize f(\x) = \begin{pmatrix}8810.0 x^5 + 5265.0 x^4 y - 35924.0 x^3 y^2 \\
%+ 76632.0 x^2 y^3 + 15717.0 x y^4 + 719.0 y^5\\
% - 164850.0 x^4 + 79194.0 x^3 y + 13391.0 x^2 y^2\\
% + 11653.0 x y^3 + 882.0 y^4 - 20358.0 x^3\\
% + 39.0 x^2 y + 709.0 x y^2 + 646.0 y^3 - 321.0 x^2\\
% - 328.0 x y + 159.0 y^2 + 2.0 x - 3.0 y\\\\\\
 %
% -6845.0 x^5 - 25334.0 x^4 y + 38860.0 x^3 y^2 \\
%- 96291.0 x^2 y^3 - 19688.0 x y^4 - 904.0 y^5 \\
%+ 200398.0 x^4 + 39751.0 x^3 y + 36049.0 x^2 y^2\\
% - 8154.0 x y^3 - 857.0 y^4 + 16382.0 x^3 \\
%- 80.0 x^2 y + 932.0 x y^2 - 635.0 y^3 \\
%- 15.0 x^2 + 28.0 x y - 82.0 y^2 - 11.0 x - 3.0 y\\
%\end{pmatrix}$$
%\end{minipage}
%\end{table*}
 %\end{figure*}
 
 %    $$\tiny f(\x) = \begin{pmatrix} 26028.8651018349 x_0^4 + 25326.9455207225 x_0^3 x_1 \\- 18233.248484753 x_0^3 + 20681.246770534 x_0^2 x_1^2 \\- 293.939966051691 x_0^2 x_1 - 191.948498819803 x_0^2 \\+ 311.301182645343 x_0 x_1^3 + 912.735390738832 x_0 x_1^2 \\- 273.692453561112 x_0 x_1\\+ 2.33199618985077 x_0 + 1026.00068010161 x_1^4 \\+ 2691.8082510703 x_1^3 \\+ 89.1776428926773 x_1^2 - 1.46324070082801 x_1 + 0.0593298154685726\\\\
 % 25969.7222728906 x_0^4 + 24898.4736614588 x_0^3 x_1 \\+ 16245.4808289768 x_0^3 \\+ 30830.4464155216 x_0^2 x_1^2 - 5219.44218205514 x_0^2 x_1 \\+ 46.748975415117 x_0^2 - 4689.24556091242 x_0 x_1^3 - 162.998536405112 x_0 x_1^2 \\- 13.607861935064 x_0 x_1 - 10.9229624231718 x_0 \\+ 187.031558402483 x_1^4 - 2007.10048997313 x_1^3 \\- 106.389868180613 x_1^2 \\- 0.372935709662556x_1 + 0.00573882572814455\end{pmatrix}$$
   
  
  
% {\bf CShape}

% \begin{tabular}{|c|c|c|cHH}                          
% \hline                              
%  & DMP & SEDS & CLFDM & CVF-CF & CVF-GS \\                    
% \hline                                                                  
% TrainingTrajectoryError & 4.40 & 8.29 & 6.90 & 8.83 & 10.62 \\         
% \hline                                                                  
% TrainingVelocityError & 7.32 & 14.73 & 12.65 & 16.94 & 21.27 \\         
% \hline                                                                  
% TestTrajectoryError & 6.99 & 9.08 & 5.82 & 10.22 & 8.83 \\             
% \hline                                                                  
% TestVelocityError & 9.43 & 12.59 & 10.89 & 19.19 & 19.63 \\             
% %\hline                                                                  
% %TrainingDTWD & 2823.14 & 15283.45 & 2472.76 & 3065.88 & 3688.03 \\      
% %\hline                                                                  
% %TestDTWD & 4514.30 & 30402.63 & 1847.63 & 3899.58 & 3927.75 \\          
% %                
% \hline                                                                  
% DistanceToGoal & 3.76 & 1.30 & 1.92 & 5.66 & 6.17 \\                    
% \hline                                                                  
% DurationToGoal & - & 3.71 & 3.39 & 4.71 & 4.12 \\                      
% \hline                                                                  
% NumberReachedGoal & 0.00 & 7.00 & 2.00 & 7.00 & 7.00 \\                 
% \hline                                                                  
% %TrainingDTWD@30T & 73380.63 & 10183.03 & 83380.79 & 1929.43 & 1912.73 \\
% %\hline                                                                  
% %TestDTWD@30T & 112357.39 & 19178.11 & 172847.69 & 3527.89 & 3323.03 \\  
% %\hline                                                                  
% GridDuration & - & 2.08 & 1.40 & 2.69 & 2.35 \\                        
% \hline                                                                  
% GridFractionReachedGoal & 0.00 & 1.0 & 0.38 & 1.00 & 1.00 \\           
% \hline                                                                  
% GridDistanceToGoal & 3.96 & 1.0 & 2.22 & 1.00 & 1.00 \\                
% \hline          
% GridDTWD & 25679.59 & 14652 & 121312.43 & 13680.30 & 12797.03 \\     
% \hline 
% TrainingTime & 0.02 & 5.34 & 6.11 & 9.56 & 7.28 \\   
% \hline                                                                  
% IntegrationSpeed & 0.21 & 0.03 & 0.04 & 0.17 & 0.06 \\
% \hline
% \end{tabular}%
% \begin{tabular}{|c|c|}
%      \hline
%      CVF-CF & CVF-GS \\
%      \hline
%      12.00 & 8.87 \\
%      \hline
%      19.93 & 15.55 \\
%      \hline
%      8.13 & 11.17 \\
%      \hline
%      11.83 & 16.40 \\
%      \hline
%      0.27 & 3.00 \\
%      \hline
%      3.00 & 3.46 \\
%      \hline
%      6.00 & 7.00 \\
%      \hline
%      1.38 & 3.33 \\
%      \hline
%      1.00 & 1.00 \\
%      \hline
%      1.00 & 1.00 \\
%      \hline
%      15251.28 & 10944.76 \\
%      \hline
%      24.59 & 24.01 \\
%      \hline
%      0.05 & 0.03 \\
%      \hline
%      \end{tabular}\CShapestats
     
% {\bf GShape}
     
% \begin{tabular}{|c|c|c|cHH}

% \hline                                                                
%  & DMP & SEDS & CLFDM & CVF-CF & CVF-GS \\                  
% \hline                                                                
% TrainingTrajectoryError & 3.81 & 7.84 & 6.41 & 7.60 & 7.54 \\         
% \hline                                                                
% TrainingVelocityError & 5.85 & 12.12 & 9.83 & 12.64 & 13.56 \\        
% \hline                                                                
% TestTrajectoryError & 5.56 & 10.44 & 11.00 & 10.84 & 7.86 \\          
% \hline                                                                
% TestVelocityError & 7.04 & 14.84 & 16.07 & 15.14 & 13.36 \\           
% \hline                                                                
% %TrainingDTWD & 2849.26 & 4304.72 & 1840.46 & 4655.76 & 2912.12 \\     
% %\hline                                                                
% %TestDTWD & 3429.42 & 5947.84 & 3095.80 & 6616.12 & 2098.42 \\         
% %\hline                                                                
% DistanceToGoal & 1.63 & 0.18 & 3.72 & 0.06 & 3.66 \\                  
% \hline                                                                
% DurationToGoal & - & 4.86 & 15.08 & 4.08 & 6.10 \\                    
% \hline                                                                
% NumberReachedGoal & 0.00 & 7.00 & 7.00 & 7.00 & 7.00 \\               
% \hline                                                                
% %TrainingDTWD@30T & 77093.83 & 4559.61 & 2995.33 & 4567.99 & 1997.90 \\
% %\hline                                                                
% %TestDTWD@30T & 87211.73 & 6374.89 & 2648.52 & 6585.13 & 1965.96 \\    
% %\hline                                                                
% GridDuration & - & 2.78 & 12.68 & 1.92 & 4.06 \\                      
% \hline                                                                
% GridFractionReachedGoal & 0.00 & 1.00 & 1.00 & 1.00 & 1.00 \\         
% \hline                                                                
% GridDistanceToGoal & 1.71 & 1.00 & 1.00 & 1.00 & 1.00 \\              
% \hline        
% GridDTWD & 19085.48 & 11493 & 10928.89 & 12522.51 & 9109.60 \\     
% \hline                                                                
% TrainingTime & 0.02 & 14.43 & 3.01 & 12.13 & 16.77 \\      
% \hline                                                                
% IntegrationSpeed & 0.18 & 0.08 & 0.10 & 0.21 & 0.04 \\   
% \hline
% \end{tabular}%
% \begin{tabular}{|c|c|}
%      \hline
%      CVF-CF & CVF-GS \\
%      \hline
%      10.07 & 6.83 \\
%      \hline
%      16.38 & 11.71 \\
%      \hline
%      5.82 & 6.29 \\
%      \hline
%      8.90 & 10.04 \\
%      \hline
%      0.18 & 0.11 \\
%      \hline
%      4.24 & 4.91 \\
%      \hline
%      7.00 & 7.00 \\
%      \hline
%      1.74 & 3.07 \\
%      \hline
%      0.94 & 1.00 \\
%      \hline
%      2.93 & 1.00 \\
%      \hline
%      17767.83 & 10637.81 \\
%      \hline
%      23.23 & 22.85 \\
%      \hline
%      0.10 & 0.03 \\
%      \hline
%      \end{tabular}\GShapestats
     

% {\bf JShape}
     
% \begin{tabular}{|c|c|c|cHH}
% \hline                                                                
%  & DMP & SEDS & CLFDM & CVF-CF & CVF-GS \\                  
% \hline                                                                
% TrainingTrajectoryError & 3.09 & 14.37 & 4.96 & 4.03 & 4.53 \\        
% \hline                                                                
% TrainingVelocityError & 6.05 & 22.88 & 9.60 & 9.53 & 10.12 \\         
% \hline                                                                
% TestTrajectoryError & 5.47 & 16.85 & 4.95 & 5.11 & 5.72 \\            
% \hline                                                                
% TestVelocityError & 8.49 & 25.76 & 9.81 & 11.40 & 12.67 \\            
% \hline                                                                
% %TrainingDTWD & 1758.26 & 6765.13 & 2666.56 & 1871.54 & 2089.53 \\     
% %\hline                                                                
% %TestDTWD & 2069.35 & 7569.03 & 3022.73 & 2841.43 & 3165.91 \\         
% %\hline                                                                
% DistanceToGoal & 2.24 & 0.00 & 6.07 & 1.68 & 3.04 \\                  
% \hline                                                                
% DurationToGoal & - & 2.05 & 3.49 & 3.58 & 3.90 \\                     
% \hline                                                                
% NumberReachedGoal & 0.00 & 7.00 & 5.00 & 7.00 & 7.00 \\               
% \hline                                                                
% %TrainingDTWD@30T & 47077.99 & 7088.01 & 7591.72 & 1430.95 & 1481.68 \\
% %\hline                                                                
% %TestDTWD@30T & 52374.65 & 7512.06 & 10253.65 & 2780.40 & 3010.00 \\   
% %\hline                                                                
% GridDuration & 100.73 & 1.21 & 2.18 & 1.56 & 2.19 \\                  
% \hline                                                                
% GridFractionReachedGoal & 0.44 & 1.00 & 0.69 & 0.94 & 0.94 \\         
% \hline                                                                
% GridDistanceToGoal & 1.42 & 1.00 & 3.61 & 3.24 & 1.55 \\              
% \hline       
% GridDTWD & 29568.10 & 12866 & 15403.52 & 23123.40 & 12021.50 \\    
% \hline                                                                
% TrainingTime & 0.01 & 18.15 & 2.66 & 23.96 & 5.62 \\   
% \hline                                                                
% IntegrationSpeed & 0.19 & 0.11 & 0.09 & 0.12 & 0.02 \\  
% \hline
% \end{tabular}%
% \begin{tabular}{|c|c|}
%      \hline
%      CVF-CF & CVF-GS \\
%      \hline
%      8.62 & 4.10 \\
%      \hline
%      14.78 & 9.31 \\
%      \hline
%      4.89 & 5.42 \\
%      \hline
%      11.28 & 11.51 \\
%      \hline
%      4.07 & 2.28 \\
%      \hline
%      3.49 & 3.79 \\
%      \hline
%      7.00 & 7.00 \\
%      \hline
%      1.56 & 3.62 \\
%      \hline
%      0.94 & 1.00 \\
%      \hline
%      3.21 & 1.00 \\
%      \hline
%      19610.23 & 10009.24 \\
%      \hline
%      22.59 & 25.20 \\
%      \hline
%      0.04 & 0.02 \\
%      \hline
% \end{tabular}\JShapestats
\normalfont


==> modulation_imgs.tex <==

\begin{figure*}[t]
    \centering
    \begin{subfigure}[t]{0.2\textwidth}
      \centering
      \includegraphics[clip, width=1\textwidth]{code/cropped_imgs/unmodulated_vectorfield}
        \caption{}
	\end{subfigure}
	\huge ${\bf \quad + \quad \alpha \quad }$\normalsize
    \begin{subfigure}[t]{0.2\textwidth}
      \centering
      \includegraphics[clip, width=1\textwidth]{code/cropped_imgs/modulation_function}
      \caption{}
	\end{subfigure}
	\huge ${\bf\quad =\quad }$ \normalsize
	\begin{subfigure}[t]{0.2\textwidth}
	  \centering
      \includegraphics[clip, width=1\textwidth]{code/cropped_imgs/modulated_angle_vf}
     \caption{}
	\end{subfigure}
	\caption{\label{fig:explain_modulation}(a) Shows a vector field $f$ learnt from a nominal path (red). (b) Depicts a repulsive vector field $\vfobstacle$ associated with an obstacle (green disk). (c) Shows modulated vector field $\tilde f$ (blue) plotted with a sample trajectory (green).}
\end{figure*}

==> new_comparisons.tex <==
\newcommand{\Anglestats}{\begin{tabular}{|c|}
\hline
CVF-P\\
\hline
6.54\\
\hline
13.93\\
\hline
4.37\\
\hline
11.45\\
\hline
2.5\\
\hline
3.34\\
\hline
7.0\\
\hline
1.88\\
\hline
1.0\\
\hline
1.0\\
\hline
1993.77\\
\hline
-1.0\\
\hline
0.01\\
\hline
\end{tabular}}

% \newcommand{\Anglestats}{\begin{tabular}{|c|}
% \hline
% Poly\\
% \hline
% 6.15\\
% \hline
% 11.73\\
% \hline
% 5.04\\
% \hline
% 10.79\\
% \hline
% 1.59\\
% \hline
% 2.92\\
% \hline
% 7.0\\
% \hline
% 1.77\\
% \hline
% 1.0\\
% \hline
% 1.0\\
% \hline
% 2172.99\\
% \hline
% -1.0\\
% \hline
% 0.13\\
% \hline
% \end{tabular}}
                       


\newcommand{\CShapestats}{\begin{tabular}{|c|}
\hline
Poly\\
\hline
10.82\\
\hline
16.83\\
\hline
17.29\\
\hline
21.06\\
\hline
nan\\
\hline
nan\\
\hline
0.0\\
\hline
nan\\
\hline
0.0\\
\hline
22.14\\
\hline
4949.96\\
\hline
-1.0\\
\hline
0.01\\
\hline
\end{tabular}}


\newcommand{\GShapestats}{\begin{tabular}{|c|}
\hline
Poly\\
\hline
8.32\\
\hline
15.11\\
\hline
9.04\\
\hline
13.49\\
\hline
3.18\\
\hline
5.91\\
\hline
3.0\\
\hline
nan\\
\hline
0.0\\
\hline
5.29\\
\hline
6279.41\\
\hline
-1.0\\
\hline
0.01\\
\hline
\end{tabular}}

\newcommand{\JShapestats}{\begin{tabular}{|c|}
\hline
Poly\\
\hline
8.84\\
\hline
15.88\\
\hline
8.01\\
\hline
13.52\\
\hline
nan\\
\hline
nan\\
\hline
0.0\\
\hline
nan\\
\hline
0.0\\
\hline
11.6\\
\hline
3120.6\\
\hline
-1.0\\
\hline
0.01\\
\hline
\end{tabular}}
